Beyond Turn-taking: Introducing Text-based Overlap into Human-LLM Interactions

Traditional text-based human-AI interactions often adhere to a strict turn-taking approach. In this research, we propose a novel approach that incorporates overlapping messages, mirroring natural human conversations. Through a formative study, we observed that even in text-based contexts, users instinctively engage in overlapping behaviors like "A: Today I went to-" "B: yeah." To capitalize on these insights, we developed OverlapBot, a prototype chatbot where both AI and users can initiate overlapping. Our user study revealed that OverlapBot was perceived as more communicative and immersive than traditional turn-taking chatbot, fostering faster and more natural interactions. Our findings contribute to the understanding of design space for overlapping interactions. We also provide recommendations for implementing overlap-capable AI interactions to enhance the fluidity and engagement of text-based conversations.

==> automatic-result-table.tex <==
\begin{table*}[t!]
\caption{OverlapBot Evaluation Results}
\label{tab:automatic-result}
    \begin{tabularx}{\textwidth}{l|>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X|>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X|>{\raggedleft\arraybackslash}X>{\raggedleft\arraybackslash}X}
    \toprule
               & \multicolumn{4}{c|}{Timing Classification} & \multicolumn{4}{c|}{Dialogue Acts Classification} & \multicolumn{2}{c}{Utterance Generation} \\
    Models    & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c}{Prec.} & \multicolumn{1}{c}{Rec.} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c}{Prec.} & \multicolumn{1}{c}{Rec.} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c}{Bleu} & \multicolumn{1}{c}{Rouge-L} \\
    \midrule
    Llama3 8B  & 0.46 & 0.50 & 0.50 & 0.46 & 0.59 & 0.79 & 0.50 & 0.37 & 0.27 & 0.11 \\
    GPT4o      & 0.50 & 0.47 & 0.47 & 0.47 & 0.73 & 0.74 & 0.76 & 0.73 & 0.08 & 0.12 \\
    GPT4 turbo & 0.50 & 0.46 & 0.46 & 0.46 & 0.75 & 0.77 & 0.77 & 0.73 & 0.26 & 0.12 \\
    \textbf{OverlapBot} & \textbf{0.67} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.85} & \textbf{0.87} & \textbf{0.78} & \textbf{0.80} & \textbf{0.48} & \textbf{0.30} \\ 
    \bottomrule
    \end{tabularx}
\end{table*}


==> table-theme.tex <==
\renewcommand{\arraystretch}{1.5} % 줄 간격 조정

\begin{table*}[t!]
\caption{Perception on OverlapBot}
\label{tab:themes}
    \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}m{2.7cm}|>{\centering\arraybackslash}m{3.3cm}|m{8cm}} % 열 너비를 조정하여 여백 제거
    \toprule
    \multicolumn{1}{c}{Main theme}                             & \multicolumn{1}{c}{Sub theme}        & \multicolumn{1}{c}{Quotes}                                                                                                                                                                                                                                                                          \\
    \midrule
    \multirow{3}{*}{\textbf{Human-like}} & Communicative    & \textit{``Unlike conventional chatbot, it felt more like having a conversation with someone who has emotions. Instead of just outputting data, it gave a stronger impression of actually conversing, so I would recommend it to someone who needs a conversational partner.'' (P16)}                     \\
                                           & Immersive        & \textit{``How I feel engaged into conversation was much better in OverlapBot, since humans used to talk in real-time for a very long time.'' (P8)}                                                                                                                              \\
    \midrule
    \textbf{Speedy Interaction}    & Efficient        & \textit{``I liked the fact that the conversation was fast-paced. I felt that the pace of the conversation was relatively quick because it started preparing responses as soon as I said something. As someone who generally prefers things to move quickly, this was a very convenient aspect.'' (P16)} \\
    \midrule
    \textbf{Brief Response}                         & Less structured & \textit{``The conventional chatbot gives more well-constructed, elaborate answers, while OverlapBot is significantly more impulsive, and the responses are catered to shorter, general responses.'' (P18)}   \\                                                              
    \bottomrule
    \end{tabularx}
\end{table*}

